TinyLidarNet: 2D LiDAR-based End-to-End Deep Learning Model for F1TENTH Autonomous Racing

Prior research has demonstrated the effectiveness of end-to-end deep learning for robotic navigation, where the control signals are directly derived from raw sensory data. However, the majority of existing end-to-end navigation solutions are predominantly camera-based. In this paper, we introduce TinyLidarNet, a lightweight 2D LiDAR-based end-to-end deep learning model for autonomous racing. An F1TENTH vehicle using TinyLidarNet won 3rd place in the 12th F1TENTH Autonomous Grand Prix competition, demonstrating its competitive performance. We systematically analyze its performance on untrained tracks and computing requirements for real-time processing. We find that TinyLidarNet's 1D Convolutional Neural Network (CNN) based architecture significantly outperforms widely used Multi-Layer Perceptron (MLP) based architecture. In addition, we show that it can be processed in real-time on low-end micro-controller units (MCUs).

==> sections/algos/h1.tex <==
\setlength{\textfloatsep}{2pt}
\begin{algorithm}[t]
\DontPrintSemicolon
\textbf{Input}:\\
Input Data ($Variable Name$),\\
\textbf{Output}: Output data\\
%\nonl\;
\SetKwProg{funct}{function}{}{}
\SetKwFunction{func}{function\_name}

\funct{\func{$Parameters$}}
{
    $var1 \gets var2$\\
    
}
\Return{$return variables$}
\caption{caption 1}
\label{alg:algo1}
\end{algorithm}

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
\fixme{remove related work and move it to introduction}
%There are several of work previously done on end-to-end networks for autonomous driving and has seen significant advancement in recent years. One of the pioneering projects and our inspiration is Dave2 architecture  \cite{Bojarski2016} was able to directly steer autonomously based on raw images as input to an end-to-end network on a real car, 2016 Lincoln MKZ on at the real road. Consequently, \cite{bechtel2018picar} faithfully recreated NVIDIA’s original CNN model for DeepPiCar. This model was then even made smaller to fit in MCU \cite{bechtel2022deeppicarmicro}. The work done by \cite{codevilla2018endtoend} utilizes input from 3 cameras to produce steering and speed outputs. The work done in  \cite{wadekar2021endtoend} uses just an image to produce steering and speed but this work is done in simulation. Other notable works are \cite{deepracer, pan2019agile}.

Previous research in the domain of end-to-end networks for autonomous driving has made remarkable progress in recent years. Among the pioneering projects that have inspired our work is the Dave2 architecture \cite{Bojarski2016}. This groundbreaking project demonstrated the capacity to directly control a real car, a 2016 Lincoln MKZ, using raw images as input to an end-to-end network, thus achieving autonomous steering on actual roads. Additionally, \cite{bechtel2018picar} recreated NVIDIA's original CNN model for DeepPiCar. Furthermore, they managed to downsize this model to make it suitable for microcontroller unit (MCU) deployment \cite{bechtel2022deeppicarmicro}, expanding the application of end-to-end networks in resource-constrained scenarios. Another notable contribution \cite{codevilla2018endtoend}, who harnessed input from three cameras to generate both steering and speed outputs, while \cite{wadekar2021endtoend} accomplished similar results using only an image, albeit within a simulated environment. Other notable works are \cite{deepracer, pan2019agile}

%2. Lidar based but objectdetections and 3D concolution or needs a backbone or it is driving
%\cite{zeng2021endtoend} utilizes lidar point cloud and an HD map at the end to end while having a backbone that takes in camera images in the backbone of the network and later does motion forecasting. \cite{casas2021intentnet} predicts intents based on LiDAR sensor, however it needs 5 to 10 lidar scans. This work as well utilizes end-to-end. \cite{evans2023highspeed} utilizes lidar values and deep reinforcement learning complete laps at high speed on 4 tracks in simulation. 
Our work addresses the limitations associated with camera-based systems by introducing Lidar as a primary sensor. They are valuable contributions in this domain as well. \cite{zeng2021endtoend} employs a combination of Lidar point cloud data and an HD map within an end-to-end framework. Interestingly, this approach incorporates Lidar in the network's backbone and motion forecasting. \cite{casas2021intentnet} focus on predicting intents based on Lidar sensor data, though they require input from 5 to 10 Lidar scans to make accurate predictions. Additionally, \cite{evans2023highspeed}  leveraging Lidar data and deep reinforcement learning to autonomously complete laps at high speeds on four different tracks within a simulation environment.  

We find the study by \cite{liu2021efficient}, "Fast Lidar Net". This model focused on lidar-based steering based on a 3D Lidar, though it did not include speed prediction. Operating on a real car, it utilized 0.64 billion Multiply-Accumulate operations (MACs) and 0.48 million parameters. It encountered difficulties when navigating sharp turns with angles of less than 90 degrees. In contrast, our model exhibited a higher level of consistency and was able to successfully navigate hairpin turns.

Moreover, our model eliminates the need to monitor the state of the vehicle, simplifying the control pipeline by directly generating steering and throttle outputs from 2D lidar scans. This design choice not only reduces computational complexity but also enhances the real-time decision-making process, making our model a competitive and efficient choice for autonomous racing.

For a more comprehensive overview of the research in this field, readers can explore additional works presented in surveys such as those by Chen et al. \cite{chen2023endtoend}, Tampuu et al. \cite{Tampuu_2022}, and Betz et al. \cite{Betz_2022}. These surveys provide an in-depth analysis of various studies and their contributions to end-to-end autonomous driving systems and racing.







%\cite{liu2021efficient} = Fast lidar net, No speed prediction but sensor faliur and steering on real car, 0.64G MACs and 0.48M////what is 47FPS mean?
%intersection 5 is particularly interesting as the model had difficulties
%completing the sharp (< 90 degree) turn angle. 
%ours made hairpin with consistency


%we don't need to know the state of our vehicle

%Surveys:
%\cite{chen2023endtoend}
%\cite{Tampuu_2022}
%\cite{Betz_2022}
%Jetson NX XAvier
% Dave Architecture
% DeepPiCar
% ESP32S3
% 
